"Thoughts & Prayers'' or ":Heart Reaction: & :Prayer Reaction:'': How the Release of New Reactions on CaringBridge Reshapes Supportive Communication During Health Crises

Following Facebook's introduction of the "Like" in 2009, CaringBridge (a nonprofit health journaling platform) implemented a "Heart" symbol as a single-click reaction affordance in 2012. In 2016, Facebook expanded its Like into a set of emotion-based reactions. In 2021, CaringBridge likewise added three new reactions: "Prayer", "Happy", and "Sad." Through user surveys ($N=808$) and interviews ($N=13$), we evaluated this product launch. Unlike Likes on mainstream social media, CaringBridge's single-click Heart was consistently interpreted as a simple, meaningful expression of acknowledgement and support. Although most users accepted the new reactions, the product launch transformed user perceptions of the feature and ignited major disagreement regarding the meanings and functions of reactions in the high stakes context of health crises. Some users found the new reactions to be useful, convenient, and reducing of caregiver burden; others felt they cause emotional harms by stripping communication of meaningful expression and authentic care. Overall, these results surface tensions for small social media platforms that need to survive amidst giants, as well as highlighting crucial trade-offs between the cognitive effort, meaningfulness, and efficiency of different forms of Computer-Mediated Communication (CMC). Our work provides three contributions to support researchers and designers in navigating these tensions: (1) empirical knowledge of how users perceived the reactions launch on CaringBridge; (2) design implications for improving health-focused CMC; and (3) concrete questions to guide future research into reactions and health-focused CMC.

==> interviewquestions.tex <==
\section{Interview Questions}\label{sec:interviewquestions}

Interviews were semi-structured; researchers asked follow-up questions not necessarily noted below. However, interviews were structured with the following base questions.

\subsection{CaringBridge Usage}
Please start by describing how you have used CaringBridge.
\begin{itemize}
    \item How long have you been using CaringBridge, and in what capacity?
     \item How often do you author posts? (How) (often)
      \item Do you have certain hopes or expectations for your posts? And/or For responses to your posts?
       \item Do you ever follow up on other people’s posts? If so, how? Do you decide between commenting, well wishes, or Reacting, and if so, how/why?
\end{itemize}


\subsection{Reaction Usage Across Social Media}
How would you say that you generally use Reactions on social media platforms? 
\begin{itemize}
    \item Do you like or dislike them? 
    \item How do they impact your experience?
\end{itemize}

\subsection{Transitioning from Single Heart Reaction to Multiple Reactions}
The “Heart” Reaction has been available for a long time on CaringBridge. In the past, how have you interpreted the meaning of using the “Heart” Reaction, when no other Reactions were available?

\begin{itemize}
    \item Do you have any stories or personal experiences about this Reaction that you would like to share?
    \item Now that there are a greater variety of Reactions available, does that change how you interpret the “Heart” Reaction? If so, how?
    \item (Possible) Are you glad CaringBridge increased the variety of reactions? Why or why not?
    \item (Possible) How do you select which Reaction to use on a given journal update?
    \item In the future, do you think CaringBridge should make even more Reactions available? What types of Reactions would you want most, and why?
\end{itemize}

\subsection{Individual Reactions}
Next, we provided an opportunity to discuss the new Reactions in more detail (“happy,” “sad,” and “prayer”). For each Reaction:

\begin{itemize}
    \item What is your opinion of this Reaction?
    \item Visitors: Have you used it yet? Why or why not?
    \item Authors: Have you received it yet? How has that made you feel?
    \item Do you have any other thoughts, concerns, or stories about this Reaction?
\end{itemize}






==> survey.tex <==

\subsection{CaringBridge Usage and Reaction Familiarity}

\subsubsection{CaringBridge Role}
Please select all of the ways that you have used CaringBridge. [Multiple choice, multiple answer]
\begin{itemize}
    \item I have contributed to authoring a CaringBridge site
    \item I have visited someone else's CaringBridge site 
    \item I have left a comment or well wish on a CaringBridge site at least once
\end{itemize}

\subsubsection{Structural Health Role}
Please select all the role(s) that currently apply to you.  [Multiple choice, multiple answer]
\begin{itemize}
    \item I am currently experiencing my own health journey or symptoms of an illness
    \item I am currently a family caregiver for someone on a health journey
    \item I am a close friend or family member of someone on a health journey
    \item I am a casual friend or acquaintance of someone on a health journey
\end{itemize}

\subsubsection{Reaction Familiarity}
How familiar are you with each of these Reactions on CaringBridge specifically? [Matrix table, single answer per row, four rows (one row per available Reaction, using an image of the Reaction as the "statement")]

\begin{itemize}
    \item I have never seen this Reaction before today.
    \item I have seen it, but never used or received it myself.
    \item I have used or received this Reaction at least once.
\end{itemize}

\subsubsection{Reaction Importance}
How important do you feel it is for CaringBridge to offer each of these Reactions? [Matrix table, single answer per row, four rows (one row per available Reaction), 3-point unipolar Likert scale] 

\begin{itemize}
    \item Not at all important
    \item Somewhat important
    \item Extremely Important
\end{itemize}

\subsubsection{Number of Available Reactions}
Do you wish CaringBridge offered even more Reaction options? [Multiple choice, single answer]

\begin{itemize}
    \item Yes, I wish CaringBridge offered even more Reaction options.
    \item No, I think these four Reaction options are sufficient.
    \item No, I think there should be fewer (or no) Reaction options.
\end{itemize}

\subsubsection{CaringBridge Email}
Please provide the email address associated with your registered CaringBridge account. [Free response]

\subsection{Questions for CaringBridge Authors}

\subsubsection{Amp Opinion}
When you think about the
\raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} symbol, to what degree do you agree with the following statements? [Matrix table, 3-point bipolar Likert responses]

\begin{itemize}
    \item The \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} is unique to CaringBridge, as opposed to other social media or emojis
    \item When my Journal update receives a \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reaction, I feel personally supported by that user
    \item I'd rather have my visitors leave an \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} than do nothing in response to my Journal updates
\end{itemize}

[Disagree | Neutral | Agree]

\subsubsection{Amp Reaction}
When you think about receiving  \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reactions on journal updates you’ve written, which of these is more important to you? [Multiple choice, single answer]
\begin{itemize}
    \item The total number of \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reactions I receive
    \item Which specific people respond with \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reactions
    \item Both of these are equally important to me
\end{itemize}

\subsubsection{Comments}
When you think about receiving comments on journal updates you've written, which of these is more important to you? [Multiple choice, single answer]

\begin{itemize}
    \item The total number of comments I receive
    \item Which specific people leave comments
    \item Both of these are equally important to me
\end{itemize}

\subsubsection{Amp Reactions vs. Comments}
If you think about receiving both  \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reactions and comments, which of these is more important to you? [Multiple choice, single answer]
\begin{itemize}
    \item Receiving \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reactions is more important to me
    \item Receiving comments is more important to me
    \item Both of these are equally important to me
\end{itemize}

\subsubsection{Desire to Receive Reactions}
Imagine you have just posted a CaringBridge journal update. Do you think you would like to receive these Reactions? [Matrix table, single answer per row, four rows (one row per available Reaction), 3-point bipolar Likert scale] 

\begin{itemize}
    \item I don't want to receive this Reaction
    \item I feel neutral about receiving this Reaction
    \item I would like to receive this Reaction
\end{itemize}

\subsection{Questions for CaringBridge Visitors}

\subsubsection{Amp Opinion (Visitors)}
When you think about the \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reaction, to what degree do you agree with the following statements? [Matrix table, 3-point bipolar Likert responses]

\begin{itemize}
    \item The \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} symbol is unique to CaringBridge, as opposed to other social media or emojis
    \item The \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} symbol is my way of saying "I support you" 
\end{itemize}

[Disagree | Neutral | Agree]

\subsubsection{Amp Frequency}
After you have read Journal update(s), how often do you feel like the following statements are true? [Matrix table, 4-point unipolar Likert responses]

\begin{itemize}
    \item I prefer to use the \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reaction instead of leaving a comment
    \item I prefer to write a comment instead of using the \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reaction
    \item I prefer to use the \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reaction and leave a comment
    \item I feel like I don't know what to write in a comment
    \item I use the \raisebox{-\mydepth}{\includegraphics[height=\myheight]{reactions/amp.jpg}} Reaction when I don't know what to write in a comment 
\end{itemize}

[Never | Rarely | Often | Always]

\subsubsection{Expectation to Use Reactions}
Imagine you are viewing a CaringBridge journal update. Do you think you will you use these Reactions? [Matrix table, single answer per row, four rows (one row per available Reaction), 3-point bipolar Likert scale] 

\begin{itemize}
    \item I won’t use it
    \item I might use it
    \item I will definitely use it
\end{itemize}

\subsection{Optional Questions for both Authors and Visitors}

\subsubsection{Choose and Describe One Reaction}
Please select just one of the Reactions below. You can make your choice for any reason—for example, based on which is your favorite (or least favorite) Reaction, or which one you have more opinions or thoughts about. [Multiple choice, single answer, responses are the four Reaction images]

Please describe why you picked this Reaction, and the type(s) of situations when you would prefer to receive (or not to receive) this Reaction on a CaringBridge Journal update. [Free response]

\subsubsection{Final Free Response} 
Do you have any last concerns or ideas about these Reactions on CaringBridge, or new Reactions that CaringBridge could introduce in the future? [Free response]

\subsection{Demographics}

\subsubsection{Gender}
What is your gender identity? (Please select one or more options.) [Multiple choice, multiple selection]

[Female | Gender nonconforming | Genderqueer | Intersex | Male | Non-binary | Trans | Something else [Free response]]


\subsubsection{Age}
What is your age? [Multiple choice, single selection] [18-24 years old | 25-34 years old | 35-44 years old | 45-54 years old | 55-64 years old | 65-74 years old | 75 years or older]


\subsubsection{Spiritual Beliefs}
How would you describe your spiritual beliefs? (Please select one or more options.)
[Multiple choice, multiple selection] [Christian | Jewish | Muslim | Spiritual, Non-Religious | Atheist | Agnostic | Something else [Free response] | Prefer Not to Say]


